Safe Balancing Control of a Soft Legged Robot

Legged robots constructed from soft materials are commonly claimed to demonstrate safer, more robust environmental interactions than their rigid counterparts. However, this motivating feature of soft robots requires more rigorous development for comparison to rigid locomotion. This article presents a soft legged robot platform, Horton, and a feedback control system with safety guarantees on some aspects of its operation. The robot is constructed using a series of soft limbs, actuated by thermal shape memory alloy (SMA) wire muscles, with sensors for its position and its actuator temperatures. A supervisory control scheme maintains safe actuator states during the operation of a separate controller for the robot's pose. Experiments demonstrate that Horton can lift its leg and maintain a balancing stance, a precursor to locomotion. The supervisor is verified in hardware via a human interaction test during balancing, keeping all SMA muscles below a temperature threshold. This work represents the first demonstration of a safety-verified feedback system on any soft legged robot.

==> Horton Balancing Paper ICRA 2023 arxiv/P00_Title.tex <==

\title{\LARGE \bf
Safe Balancing Control of a Soft Legged Robot}

\author{Ran Jing$^{1}$, Meredith L. Anderson$^{1}$, Miguel Ianus-Valdivia$^{1}$, Amsal Akber Ali$^{1}$, Carmel Majidi$^{2}$,\\ Andrew P. Sabelhaus$^{1,3}$% <- stops a space
\thanks{This work was in part supported by the Office of Naval Research under Grant No. N000141712063 (PM: Dr. Tom McKenna), the National Oceanographic Partnership Program (NOPP) under Grant No. N000141812843 (PM: Dr. Reginald Beach), and an Intelligence Community Postdoctoral Research Fellowship through the Oak Ridge Institute for Science and Education.}
\thanks{$^1$R. Jing, M.L. Anderson, M. Ianus-Valdivia, A. Akber Ali and A.P. Sabelhaus are with the Department of Mechanical Engineering, Boston University, Boston MA, USA. {\tt\small \{rjing, merland, maiv, aakber, asabelha\}@bu.edu} }
% \thanks{$^2$A.P. Sabelhaus was with the Department of Mechanical Engineering, Carnegie Mellon University, Pittsburgh PA, USA. He is now with }
\thanks{$^2$C. Majidi is with the Department of Mechanical Engineering and the Robotics Institute, Carnegie Mellon University, Pittsburgh PA, USA. {\tt\small cmajidi@andrew.cmu.edu}}
\thanks{$^3$A.P. Sabelhaus is also with the Division of Systems Engineering, Boston University, Boston MA, USA.}
% \author{Albert Author$^{1}$ and Bernard D. Researcher$^{2}$% <-this % stops a space
% \thanks{*This work was not supported by any organization}% <-this % stops a space
% \thanks{$^{1}$Albert Author is with Faculty of Electrical Engineering, Mathematics and Computer Science,
%         University of Twente, 7500 AE Enschede, The Netherlands
%         {\tt\small albert.author@papercept.net}}%
% \thanks{$^{2}$Bernard D. Researcheris with the Department of Electrical Engineering, Wright State University,
%         Dayton, OH 45435, USA
%         {\tt\small b.d.researcher@ieee.org}}%
}

% , 

\maketitle
\pagestyle{empty}  % no page number for the second and the later pages
\thispagestyle{empty} % no page number for the first page

==> Horton Balancing Paper ICRA 2023 arxiv/P0_Abstract.tex <==

\begin{abstract}

Legged robots constructed from soft materials are commonly claimed to demonstrate safer, more robust environmental interactions than their rigid counterparts.
However, this motivating feature of soft robots requires more rigorous development for comparison to rigid locomotion.
This article presents a soft legged robot platform, Horton, and a feedback control system with safety guarantees on some aspects of its operation. 
The robot is constructed using a series of soft limbs, actuated by thermal shape memory alloy (SMA) wire muscles, with sensors for its position and its actuator temperatures.
A supervisory control scheme maintains safe actuator states during the operation of a separate controller for the robot's pose.
Experiments demonstrate that Horton can lift its leg and maintain a balancing stance, a precursor to locomotion.
The supervisor is verified in hardware via a human interaction test during balancing, keeping all SMA muscles below a temperature threshold.
This work represents the first demonstration of a safety-verified feedback system on any soft legged robot.
\end{abstract}

% \begin{IEEEkeywords}
% control
% \end{IEEEkeywords}


==> Horton Balancing Paper ICRA 2023 arxiv/P1_Introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Outline:

% P1 = motivation overview, grand challenges. Soft robot locomotion, purposes of locomotion, control vs. rigid robots (limitations of past soft robots)

% P2 = this work, description of primary findings/claims, its contributions toward grand challenges. Ref Fig 1. Robot that can balance, precursor to walking, with full body control and some safety guarantees

%% 1.2 Robot Locomotion, Soft and Rigid

% P1 = gaits and balancing
% P2 = soft robots don't do that. Horton is the first to have enough sensing, actuation, and corresponding control infrastructure for controlling the entire pose of a soft legged robot.

%% 1.3 Safety-based control

% P1 = importance of safety. Done a lot for rigid robot, soft just informal.
% P2 = our approach to safety.

%% 1.4 Contributions

% Three bullet points of specific contributions


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
Locomotion of robots built from soft and compliant materials has the potential to expand exploration efforts in extreme, delicate, or dangerous locations that are unsafe or difficult to reach for either humans or traditional rigid robots \cite{Rus_Tolley_2015,Calisti_fundamentals_2017}. 
However, the source of these robots' benefits -- conforming to unstructured environments and unanticipated disturbances -- introduces significant challenges in control, modeling, and mechanical design \cite{Rich_untethered_2018}.
Most soft robot locomotion has been limited to simple motions in open-loop \cite{scott_geometric_2020,Huang2019,patterson_untethered_2020,bern_trajectory_2019}, a stark contrast to the intelligent full-body control of rigid systems \cite{ames_rapidly_2014}, which often come with provable performance properties.

% Something about soft robots having limited methods of locomotion and control, a far cry from state-of-the-art in rigid robot walking.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/horton_balencing_v4.pdf}
    \caption{The soft legged robot Horton demonstrates dynamic balancing motions, and full pose control, using feedback with some formal safety verification.}
    \label{fig:horton_balancing}
    \vspace{-0.3cm}
\end{figure}

This article makes progress in bridging the gap.
We introduce a soft legged robot, Horton, with sufficient actuation, sensing, and feedback to demonstrate dynamic balancing (Fig. \ref{fig:horton_balancing}).
Horton's feedback control framework includes a safety verification for its most failure-prone component, the shape memory alloy (SMA) artificial muscles.
This is the first framework and experimental validation of full pose control with any verifiable safety for any soft legged robot, using dynamic balancing as a precursor to future walking locomotion \cite{ott_posture_2011}.

% In a step towards expanding exploration capabilities through the practical implementation of soft robotic locomotion, we propose a soft robot capable of balancing and maintaining a pose. By integrating powerful actuation with proprioceptive sensing in a simplified limb design, this system represents the first soft legged robot equipped with closed-loop feedback control for verifiable safety. 
% \fix{transition to information about previous work and horton design specs}

% Where traditional rigid robots lack compliance, soft robots are capable of deforming to their environment and recovering their initial shape \cite{Rus_Tolley_2015}. 
% However, locomotion requires exerting force on the environment to generate motion, which is at odds with the deformable nature of soft robots. 
% This presents challenges in actuation and control that hinders progress towards practical implementation of a soft walking robot that retains meaningful functionality \cite{Calisti_fundamentals_2017}. 

\begin{figure*}[t]
    \centering
    \includegraphics[width = \textwidth]{figures/hardware_and_system-horizontal.pdf}
    \caption{The Horton robot platform contains five SMA-actuated limbs arranged for planar motions (a), connected via 3D-printed brackets (b) with temperature sensors (b)(1) connected to the two SMAs per-limb (b)(2) alongside sensors for bending angle (b)(3). The robot's feedback system operates on an adjacent computer and microcontroller (c), which controls the angles $\theta_1 \hdots \theta_5$ of each of the five limbs (d). The ten corresponding SMAs are labeled according to leg/spine segment ($L_i/S_i$) and direction of induced bending ($+/-$).}
    \label{fig:horton_hardware_and_system_architecture}
    \vspace{-0.5cm}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Robot Locomotion and Control, Soft or Rigid}

Mobile soft robots rely on the elastic deformation of their bodies for locomotion \cite{Calisti_fundamentals_2017}, often preventing the use of full state feedback while also limiting versatility.
Friction-based gaits such as crawling \cite{Tolley_quadrupedal_2014,Schiller_gecko_2020,Onal_snake_2013,Thomas_inchworm_2021} rely on continuous contact with the ground for stability, resulting in slow locomotion and inability to overcome obstacles of larger sizes.
Jumping motions are inherently limited in the accuracy of their landing location \cite{tolley_untethered_2014,Mintchev2018,Huang2019}.
Progress toward controlled soft locomotion has therefore focused on legged robots, but prior work has either been restricted to aquatic environments for stability \cite{Cianchetti_OCTOPUS_2015,Calisti_Poseidrone_2015,patterson_untethered_2020} or been limited with speed and unverified feedback approaches \cite{Li_modular_2022}.

% such as crawling, jumping, and legged locomotion\cite{Calisti_fundamentals_2017}. 
% Mobile soft robots leverage a variety of approaches to locomotion, such as crawling, including two-anchor, peristaltic, and serpentine crawling, jumping, and legged locomotion, including hopping, running, and walking \cite{Calisti_fundamentals_2017}. 
% Many state of the art mobile soft robots use variations of a crawling gait, including a pneumatic quadrupedal soft robot \cite{Tolley_quadrupedal_2014} and several soft robots inspired by animals, such as a gecko \cite{Schiller_gecko_2020}, snake \cite{Onal_snake_2013}, and inchworm \cite{Thomas_inchworm_2021}. 
% However, friction based gaits, like crawling, are some of the slowest approaches to generating locomotion \cite{Calisti_fundamentals_2017}. 
% These types of gaits rely on continuous contact with the ground for stability, which inherently limits their versatility in adapting to unstructured environments. 
% Investigating soft robotic locomotion is widely considered to have the ultimate goal of expanding exploration capabilities in inaccessible, dangerous, or unstructured locations where the environmental conditions might be largely unknown \addref. 
% Approaches to locomotion, including friction-based gaits, that lose functionality outside of preferred environmental conditions are fundamentally limited in their ability to make progress towards practical implementation. 

In contrast, rigid legged robots can typically locomote over large environmental obstacles, in structured or semi-structured environments \cite{lee_learning_2020}.
Since dynamic balancing and locomotion are unstable, feedback control over the robot's entire pose is required \cite{majumdar_control_2014}.
Bringing these capabilities to soft robots will require new architectures that can execute similar control systems.

% Combining the terrain navigation capabilities of rigid legged robots with the benefits of compliance will require designs and control systems that bring similar algorithms to soft legged robots.

% However, the dynamic gaits necessary for legged locomotion are unstable.
% In order to bring the benefits of compliance to the capabilities of rigid robots, new approach are required to design and control. 
% Dynamic locomotion necessitates dynamic feedback, which in turn requires sufficient sensing and actuation...

% Legged locomotion that involves lifting a leg, or removing ground contact, to take a step is not subject to the same restrictions as friction-based gaits for overcoming obstacles.
% However, the dynamic gaits necessary for legged locomotion are unstable. 
% Just taking a step requires a significant force output and robust control in order to lift and precisely reposition a leg while simultaneously supporting the body and maintaining balance. 
% As such, soft robots that use legged locomotion have seen greater success for underwater exploration as compared to exploration on dry land. 
% For instance, the soft eight-arm OCTOPUS robot \cite{Cianchetti_OCTOPUS_2015} and the octopus-inspired PoseiDRONE \cite{Calisti_Poseidrone_2015} are capable of executing dynamic motions at a greater speed, but their functionality is predicated on external support from an underwater environment. 

% While limitations in soft robotic actuation and control pose significant challenges, the key to a successful soft robot with versatile legged locomotion is stability. The robot must maintain balance, providing compliance when desired and structure when needed. Where imprecise limb motions are sufficient for the aforementioned friction-based gaits, balancing for legged locomotion requires executing motions in real time that accurately and consistently achieve and maintain desired configurations. Notably, systems lacking feedback about their state presuppose safety based on the emboddied intelligence inherent in soft materials. However, this assumption alone is insufficient to rigorously verify safety during unmodeled interactions, both for the robot itself and for the surrounding environment or humans it comes into contact with. Approaches to locomotion in which functionality relies on assumptions about the surrounding environment and about the safety of interactions are at risk of failure when those assumptions fall apart. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Control and Safety}

State-of-the-art locomotion of rigid robots has been enabled by feedback control with verifiable properties, such as stability of hybrid systems \cite{sreenath_compliant_2011} and invariance \cite{ames_rapidly_2014}.
% Both approaches prove conditions on robot states converging to a desired value, or remaining with in an acceptable range.
Set invariance formally defines safety: if a robot's states remain within some set for all time under the action of feedback, its operation is safe \cite{gilbert_linear_1991,blanchini_set_1999}.
In contrast, stable soft robot controllers have only been shown for manipulation \cite{della_santina_model-based_2020,della_santina_control_survey}.

% Describe the concept of invariance re: safety and how rigid robot locomotion uses it sometimes, how relates to the control barrier function stuff

% However, closed-loop feedback control of soft robots is complicated by the inherent properties of soft materials \cite{della_santina_control_survey}. 
% Deformable materials of infinite dimension are incredibly difficult to model with both simplicity and accuracy while accounting for dynamic motion. 
% A variety of approaches have been employed in an attempt to simplify feedback control for soft robots.
% \fix{more about soft robot control approaches?/past papers with verifiable safety (touched on in system model section)}

Since balancing and locomotion involve environmental interaction, disturbances and unmodeled contact are major failure modes.
Soft robots, though informally `safe' by way of limiting their forces or positions \cite{lasota_survey_2017,tonietti_design_2005}, commonly use novel actuators \cite{zhang_robotic_2019} with possible catastrophic failure modes in these situations.
Under a strong disturbance, Horton's thermoelectric SMA actuators would overheat \cite{soother_challenges_2020} and fail, as would equivalent designs using pneumatics (bursting \cite{terrynSelfhealingSoftPneumatic2017}) and dielectrics (electrical breakdown or arcing \cite{planteLargescaleFailureModes2006,bilodeauSelfHealingDamageResilience2017}). 
As of yet, approaches for safer operation of soft robots of any type have relied on simple hard stops \cite{villanuevaBiomimeticRoboticJellyfish2011,coloradoBiomechanicsSmartWings2012,whiteSoftParallelKinematic2018,yeeharntehArchitectureFastAccurate2008}, with only limited examples of intelligent shutoff \cite{balasubramanian_fault_2020}.

% Verified control for soft locomotion may therefore be as much about invariance as it is about stability.
% However, stuff about soft robots not doing so well with that, again mostly relying on design.

% In a step towards expanding exploration capabilities through the practical implementation of soft robotic locomotion, we propose a soft robot capable of balancing and maintaining a pose. By integrating powerful actuation with proprioceptive sensing in a simplified limb design, this system represents the first soft legged robot equipped with closed-loop feedback control for verifiable safety. 
% \fix{transition to information about previous work and horton design specs}

% Safety stuff - Temperature supervisor \cite{sabelhaus_safe_2022}.
% SMAs paragraph.
% high work density \cite{Rich_untethered_2018}.
% Previous robots .

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.1cm} % hack for space
\subsection{Contribution}

% SMA high work density \cite{Rich_untethered_2018}

% This work presents a soft legged robot with the actuation, sensing, and feedback to perform verifiably-safe motions.

% The Horton robot architecture (Fig. \ref{fig:horton_hardware_and_system_architecture}) contributes multiple advances toward soft robot balancing and locomotion.
The Horton architecture (Fig. \ref{fig:horton_hardware_and_system_architecture}) contributes a platform particularly well-suited to studying balancing control and safety in soft robots.
Horton uses SMA-powered limbs to create high forces, strains, and speeds due to their work density \cite{Rich_untethered_2018}, extending prior work in soft limb design \cite{walters2011digital,wertz_trajectory_2022,patterson_robust_2022,patterson_untethered_2020,sabelhaus_-situ_2022}.
Consequently, Horton has dynamic motions and the associated instabilities that motivate control research in rigid legged robots.
This work applies a supervisory controller to Horton's SMAs during pose control, adapted for multiple soft limbs from prior work \cite{sabelhaus_safe_2022}.
Specifically, this article contributes:

\vspace{0.1cm}
\begin{tightenumerate}
    \item A soft robot legged robot platform with sufficient state sensing and actuation for full pose control,
    \item The first application of a verifiably-safe controller to a soft legged robot, and
    \item A demonstration of safe balancing motions during an otherwise-unsafe disturbance test.
\end{tightenumerate}

% This work applies the previously derived controller for the first time
% The designs in this work use the same design and prototyping framework as the previous article and can be considered an application of these approaches to a legged robot



==> Horton Balancing Paper ICRA 2023 arxiv/P2_Robot_Architecture.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-0.1cm} % hack for space
\vspace{0.1cm}
\section{Robot Architecture}

Horton is constructed from five soft limbs, arranged to create planar motions, with pairs of antagonistically-arranged SMA wire coils (Fig. \ref{fig:horton_hardware_and_system_architecture}(a),(b)) that produce bidirectional bending (Fig. \ref{fig:horton_hardware_and_system_architecture}(d)).
This simple planar design facilitates the development of fundamental control results for soft legged robots.
The robot is also connected to a tether for power and communication (Fig. \ref{fig:horton_hardware_and_system_architecture}(a)), oriented upward from the center of the body, with loose cables.
% The tether did not artificially assist in balancing, as the robot was observed to often fall during initial experiments.
Though the tether may exert some external forces on the robot, those forces were not sufficient to achieve dynamically stable balancing -- i.e., the robot was often observed to fall during initial experiments.

% We connect the robot to a tether for power and communications, \fix{but that's not a big deal.}
% The walking robot used in these experiments is constructed using five 1-DOF limbs, each capable of actuating in either direction from the origin, measuring the temperature of both SMA actuators, and bending angle all in real-time. 

% Due to the robots need for large amounts of power, the robot remains tethered to a power source. As shown in Figure \ref{fig:horton_balancing}, the tether is oriented upwards from the center of the body. Even in this configuration, we found the tether to provide no support to the robot, as the robot has been noted to fall in both powered and resting states. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mechanical Design, Actuation, and Sensing}

The soft limbs used in Horton are adapted from a prior design \cite{sabelhaus_-situ_2022}, now with 3D-printed brackets to connect them.
The molded body of the limb (Smooth-Sil 945, Smooth-On) houses the two SMA springs (Dynalloy Flexinol $90^\circ$C, 0.020'' diam.) in slotted compartments, allowing rapid convective cooling. 
% The SMAs are placed in an antagonistic configuration, actuating the limb about its most flexible axis. 
Attached to the end of each SMA is a thermocouple (5TC-TT-K-36-72, Omega), affixed using thermally conductive, electrically insulating epoxy. 
A soft capacitive angular displacement sensor (Bendlabs 1-axis) is inserted along a slot in the side of the limb.
% The sides of the silicone body incorporate slots which house a soft angular displacement sensor (1-Axis Soft Flexible Sensor, Bend Labs). 

The SMAs are powered individually by MOSFETs connected to a 7V power supply, controlled by pulse width modulation voltage signals $\bu(k) \in [0,1]$ from a microcontroller. 
Pulling the MOSFETs high creates a current through the SMA, causing contraction due to Joule heating. 
The microcontroller sends temperature and bend angle measurements to a computer, which in turn specifies PWM duty cycle (Fig. \ref{fig:horton_hardware_and_system_architecture}(c)).
% Distributing the correct signals to the SMA's, collecting, and formatting all of the data, are tasks completed by an Arduino Mega, providing an interface between the robot and the computing. 
% The computations are all performed on a laptop computer in Python, and sent back to the Arduino for distribution.

% The limbs are attached to each other using a tab of material molded onto the limb secured to a lightweight 3D printed bracket. The configuration of the legs results in a flexible robot composed of two spine segments and three legs. All of the limbs are placed with their bending axes in line, resulting in a summative motion of the limbs in a single plane.

% Feedback from the soft angular displacement sensor about the bending degree $\theta_i$ of each limb can be used to estimate the robot's pose according to a constant curvature assumption \cite{Webster_CC_2010}. \fix{not sure where this sentence should go}

This article takes the robot body's state space as the set of angles $\bq = \begin{bmatrix}\theta_1 & \hdots & \theta_5\end{bmatrix}^\top$, Fig. \ref{fig:horton_hardware_and_system_architecture}(d).
Prior work has shown how tip-tangent angle readings of capacitive bend sensors $\alpha_i$ can be converted into bending angles $\theta_i$ via assumption of piecewise constant curvature (PCC) \cite{toshimitsu_sopra_2021,wertz_trajectory_2022,patterson_robust_2022}.
If PCC holds, $\theta_i = \alpha_i/2$.
Horton's operation departs substantially from PCC.
However, we focus on proof-of-concept balancing in \textit{any} pose while leaving kinematic tracking for future work.

\subsection{System Architecture}

% \fix{The software has a few different components.
% Data flows this way and that way.}

Controller calculations occur on a laptop (Core i5, 2.6 GHz, 16 GB RAM) attached to an Arduino Mega microcontroller (Fig. \ref{fig:horton_hardware_and_system_architecture}(d)).
In this framework, sensor readings include both pose states $\bq(k)$ and other internal states $\bx(k)$, which here are the robot's SMA temperatures.
% t any $k$, sensor readings of joint angles $\bq(k)$ and other robot state variables $\bx(k)$ such as the SMA's temperature are filtered and sent to the controller. 
At time $k$, a controller for the robot's pose calculates an input signal $\bu(k)$ intended to regulate the robot around a specified setpoint $\bar\bq(k)$, which is passed through the supervisor to get the safety-guaranteed PWM signal $\hat\bu(k)$, inducing heating current $\mathcal{I}$.
The following section details the signals and computations, including the proportional-integral controller with anti-windup (PIAW) for pose control.
This architecture is generalizable to other soft legged robots with actuator dynamics.

% The controller gets the output $\bu(k)$ and sent it to the safety supervisor. 
% Then, the supervisor considers system constraints and current robot state $\bx(k)$ to get the safety-guaranteed output $\hat \bu(k)$. 
% Finally, limited output $\hat \bu(k)$ is converted to the heating current $\mathcal{I}$ by Arduino's pulse-width modulation (PWM) generator. \fix{In here or hardware, explain PWM - RMS in current - bending angle in the limb.}
% \fix{Phase the following better.}To address the supervisor's saturating problem, we implement a proportional-integra controller with anti-windup functionality (PI-AW). 
% It takes the current joint state $\bq(k)$, setpoints, and actual control output from the last step $\hat \bu(k-1)$ to determine the output $\bu(k)$ before supervising. 
% Calculations in the supervisor and P-IAW blocks are described in the following section. 
% This control system architecture is generalizable for any soft legged robot.



% The overall control system architecture is shown in Fig. \ref{fig:horton_hardware_and_system_architecture}c. 
% As described in the previous section, logically our system has three units, a python script running on PC as the controller, a microcontroller (Arduino Mega) as the signal processing unit, and Horton as the soft legged actuator.

==> Horton Balancing Paper ICRA 2023 arxiv/P3_Math.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Supervisory Control for Soft Legged Robots}

The robot presented here experiences unsafe operation of its actuators under disturbances.
A simple on/off hard stop on temperature causes chatter.
Instead, this article's supervisory control system dynamically saturates the input signal to maintain a provable safety specification.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{System Model}

Soft robots are highly nonlinear systems in general \cite{della_santina_control_survey}, and many state parameterizations exist for the dynamics of soft bodies and actuators \cite{goury_fast_2018,della_santina_model-based_2020,huang_dynamic_2020}.
The most common model-based representations for control \cite{armanini_soft_2021} result in a system of ordinary differential equations, which we assume are discretized appropriately:

\begin{equation}
    \bz(k+1) = f(\bz(k), \bu(k))
\end{equation}

\noindent with states $\bz \in \mathbb{R}^N$ and inputs $\bu \in \mathbb{R}^P$.

This article focuses on a subset of these states $\bx \in \mathbb{R}^M$ for which safety concerns exist, as in $\bz = [\bq^\top \; \bx^\top]^\top$.
In the Horton robot, the states $\bx = \begin{bmatrix} T_1 & \hdots & T_m \end{bmatrix}^\top$ are the SMA wire temperatures, which will readily exceed a safe limit under feedback architectures that do not account for disturbances.
We leave the body dynamics safety in $\bq$ for future work.

It has been established that the temperature dynamics of SMA wires are accurately approximated by thermal models for Joule heating \cite{mollaei2012optimal,katoch2015trajectory,bhargaw2013thermo,cheng2017modeling,wertz_trajectory_2022,sabelhaus_safe_2022}, which for this study takes the form of a scalar affine system:

\begin{equation}
    T_i(k+1) = -\frac{h_c A_c}{C_v}(T_i(k) - T_0)\Delta_t + \frac{1}{C_v} \Delta_t P_i(k)
\end{equation}

\noindent with input power represented in terms of a pulse-width modulation input $u_i(k) \in [0,1]$ as $P_i(k) = \rho J^2 u_i(k)$.
Here, $h_c$, $A_c$, $C_v$, $\rho$, and $J$ are various constants for material, geometry, and electrical properties, all fixed scalars.
Lumping all unknown constants produces

\begin{equation}
    T_i(k+1) = a_{(1,i)} T_i(k) + a_{(2,i)} u_i(k) + a_{(3,i)}.
\end{equation}

\noindent We assume that $\{a_1, a_2, a_3\}$ will be fit from hardware data on SMA temperature and duty cycle as in prior work \cite{wertz_trajectory_2022}.

Lastly, we transform this system of scalar affine equations into one linear system. 
Augmenting the states with a brief abuse of notation as $\bx_i = \begin{bmatrix} T_i & 1 \end{bmatrix}^\top \in \mathbb{R}^2$ gives each wire's dynamics as $\bx_i(k+1) = \bA_i \bx_i(k) + \bB_i u_i(k)$, where $\bA = [ a_{(1,i)}, \; a_{(3,i)}; \; 0, 1] \in \mathbb{R}^{2 \times 2}$ and $\bB = \begin{bmatrix} a_{(2,i)} & 0 \end{bmatrix}^\top \in \mathbb{R}^2$.
Arranging into one system $\bx(k+1) = \bA \bx(k) + \bB \bu(k)$ produces a block structure:

\begin{equation}\label{eqn:linsys_block}
    \bx(k+1) = \begin{bmatrix}
        \bA_1 & & \\
        & \ddots & \\
        & & \bA_m
    \end{bmatrix} \bx(k) + \begin{bmatrix}
        \bB_1 \\ \vdots \\ \bB_m
    \end{bmatrix} \bu(k).
\end{equation}

\noindent We use eqn. (\ref{eqn:linsys_block}) in most of the remainder of the article to drop the $i$-indexing.
% , while noting that \fix{something about how results could be derived individually so no one should freak out about the matrix inverses later}.

% \begin{figure*}[tb]
%     \centering
%     \includegraphics[width=\textwidth,height=5.5cm]{figures/foot_height_v5.pdf}
%     \caption{The figure shows the foot height of Horton's lifted front leg during the experiment. The foot height is the distance from the center of the red dot mark to the surface of our testbed. We artificially divide the process into four stages (a)-(d). A typical snapshot of Horton's posture at each stage is presented above.}
%     \label{fig:horton_foot_height}
% \end{figure*}

% \begin{figure*}[tb]
%     \centering
%     \begin{subfigure}[h]{1\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/foot_height_v5.pdf}
%         \caption{The figure shows the foot height of Horton's lifted front leg during the experiment. The foot height is the distance from the center of the red dot mark to the surface of our testbed. We artificially divide the process into four stages (a)-(d). A typical snapshot of Horton's posture at each stage is shown in the upper of the figure.}
%         \label{fig:horton_foot_height}
%     \end{subfigure}
%     %\vspace here if needed
%     \begin{subfigure}[h]{1\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/horton_state_v3.pdf}
%         \caption{(a) The actual bending angle $\theta$ and the setpoint of each limb during the experiment. (b) The temperature limit of SMA $T^{max}$ and temperature readings of all 10 SMAs. 3 of them are highlighted for experimental analysis. (c) The PWM output (in percentage) that applied to each SMA during the experiment. SMAs that are highlighted in (b) are also highlighted in (c).}
%         \label{fig:horton_state}
%     \end{subfigure}
%     \label{fig:horton_experiments}
% \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Supervisor's Saturating Controller}

This work assumes the desired safety condition is pre-specified as a bound on $\bx$.
For Horton, bounds are a maximum temperature $T^{MAX}$, and we seek to guarantee that $\bx_i(k) \leq \begin{bmatrix} T^{MAX} & 1 \end{bmatrix}^\top$ $\forall k \in \mathbb{N}^+$, i.e., $\bx(k) \leq \bx^{MAX}$.
The following section adapts our recent result which does so \cite{sabelhaus_safe_2022}, now for a robot with multiple SMA-powered limbs (eqn. (\ref{eqn:linsys_block})).

Consider first the standard result \cite{baggio_data-driven_2019} that a linear system can be driven from $\bx(k)$ to a setpoint $\bx^{SET}$ in $K$-many steps, given reachability conditions, via the minimum-energy control sequence $\bu^*(k) = \bB^\top (\bA^\top)^{K-k-1} \bW_K^\dag (\bx^{SET} - \bA^K \bx(k))$, where $\bW_K$ is the $K$-step controllability Grammian \cite{baggio_data-driven_2019,sabelhaus_safe_2022}.
Taking a one-step ahead window $K=k+1$ as a worst case, with shortest time to reach $\bx^{SET}$,

\begin{equation}\label{eqn:onestep_set}
    \bu^*(k) = \bB^\top (\bB \bB)^\dag (\bx^{SET} - \bA \bx(k)).
\end{equation}

The system in eqn. (\ref{eqn:linsys_block}) is monotone \cite{sabelhaus_safe_2022}, so applying $\bu(k) \leq \bu^*(k)$ guarantees that $\bx(k+1) \leq \bx^{SET}$ elementwise.
Intuitively, applying less current generates lower wire temperatures.
However, to make this approach more robust, we propose to constrain inputs to some fraction of the setpoint amount, $\bu(k) \leq \gamma \bu^*(k)$, where $\gamma \in (0,1)$.
Our prior work showed that maintaining this condition in a closed loop changes the desired equilibrium point \cite{sabelhaus_safe_2022}, and so to obtain $\bx^{MAX}$ as the constraint, the following adjustment is required of the setpoint:

\begin{equation}\label{eqn:setpoint_adjust}
    \bx^{SET} = \left( 1 / \gamma \right) \left(\bI - \left(1 - \gamma \right) \bA \right) \bx^{MAX}.
\end{equation}

\noindent We combine eqns. (\ref{eqn:onestep_set})-(\ref{eqn:setpoint_adjust}) with feedback of $\bx(k)$,

\begin{align}\label{eqn:umax}
    \bu(\bx(k))^{MAX} & = \gamma \bB^\top (\bB \bB^\top)^\dag ( \left( 1 / \gamma \right) (\bI \; \hdots \notag \\
    & - \left(1 - \gamma \right) \bA)  ) \bx^{MAX} - \bA \bx(k) ).
\end{align}

The closed loop system obtained with $\bu(\bx(k)) = \bu(\bx(k))^{MAX}$ can be written in terms of the error $\be(k) \defeq \bx(k) - \bx^{MAX}$ as $\be(k+1) =\gamma \bA \be(k)$, which is exponentially stable under easily anticipated conditions.
However, that does not necessarily guarantee $\bx(k) \leq \bx^{MAX} \; \forall k$, which corresponds to $\be(k) \leq 0$.
To verify this safety property, we prove that the set of states $\mathcal{S} = \{\be \; | \; \be \leq 0\}$ is invariant under the closed-loop dynamics; i.e., $\be(0) \leq 0 \Rightarrow \be(k) \leq 0 \; \forall k \in \mathbb{N}^+$.
Noting that $\mathcal{S}$ is a polyhedron, it is invariant \cite{gilbert_linear_1991,blanchini_set_1999} under the transition matrix $\gamma \bA$ if $\mathcal{S} \subseteq \{ \be \; | \; \gamma \bA \be \leq 0\}$. 
That condition can also be written using set equivalence, 

\begin{equation}\label{eqn:S_invariance}
    \mathcal{S} \cap \{ \be \; | \; \gamma \bA \be \leq 0\} = \mathcal{S}.    
\end{equation}

Calculations from prior work \cite{sabelhaus_safe_2022} showed that eqn. (\ref{eqn:S_invariance}) held true for all experimentally-calibrated SMA thermal dynamics models, and therefore $\mathcal{S}$ is invariant.
We refer the reader to the literature for further discussions concerning the $Pre$ operation implied in eqn. (\ref{eqn:S_invariance}) and maximum invariant set calculations \cite{gilbert_linear_1991,blanchini_set_1999,sabelhaus_safe_2022}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Incorporating Pose Feedback and Verifying Safety}

Operating the robot using $\bu(\bx(k)) = \bu(\bx(k))^{MAX}$ maintains safe temperatures but does not allow for controlling the pose of the robot, i.e. the other states in $\bz$.
Instead, assume that there is another feedback controller $\bv(\bz(k))$ developed independently, which we would like to operate unless it would lead to unsafe states.
Propose the following (elementwise) composition, recalling that $\bx$ is part of the full state $\bz$,
% \fix{decide if we're OK switching out the argument from x to z as needed}

% \begin{equation}\label{eqn:awesome_controller}
%     \hat u_i(\bz(k)) = \begin{cases}
%         v_i(\bz(k)) & \text{if} \quad v_i(\bz(k)) \leq u_i(\bx(k))^{MAX} \\
%         u_i(\bx(k))^{MAX} & \text{else}
%     \end{cases}
% \end{equation}

\begin{equation}\label{eqn:awesome_controller}
    \hat u_i(\bz(k)) = \begin{cases}
        v_i(\bz(k)) \quad \; \; \; \text{if} &  v_i(\bz(k)) \leq u_i(\bx(k))^{MAX} \\
        u_i(\bx(k))^{MAX} & \text{else}
    \end{cases}
\end{equation}

The closed loop system under $\hat \bu(\bz(k))$ has the same invariance properties, and therefore safety, as the dynamics under solely $\bu(\bx(k))^{MAX}$. 
Formally:

\begin{theorem}
    The set $\mathcal{S} = \{\be \; | \; \be \leq 0 \}$ is invariant for the closed loop system obtained by applying $\hat\bu(\bz(k))$ to the dynamics of eqn. (\ref{eqn:linsys_block}) if invariance under $\bu(\bx(k))^{MAX}$ has been verified via eqn. (\ref{eqn:S_invariance}).
\end{theorem}

\begin{proof}
    Consider any state $\bx_i(k) \leq \bx_i^{MAX}$, i.e. $\be(k) \in \mathcal{S}$. Since $\mathcal{S}$ is invariant under the supervisor alone, $\bA_i \bx_i(k) + \bB_i \bu_i(\bx(k))^{MAX} \leq \bx_i^{MAX}$.
    Then since eqn. (\ref{eqn:linsys_block}) is a monotone control system and by definition of $\hat\bu$ in eqn. (\ref{eqn:awesome_controller}),

    \begin{align}
        \hat \bu_i(\bz(k)) & \leq \bu_i(\bx(k))^{MAX}, \notag \\
        \bA_i \bx_i(k) + \bB_i \hat \bu_i(\bz(k)) & \leq \bA_i \bx_i(k) + \bB_i \bu_i(\bx(k))^{MAX}, \notag \\
        \bA_i \bx_i(k) + \bB_i \hat \bu_i(\bz(k)) & \leq \bx_i^{MAX}, \notag \\
        \therefore \bx_i(k+1) & \leq \bx_i^{MAX}, \notag
    \end{align}

    \noindent so $\be(k+1) \in \mathcal{S}$, and $\mathcal{S}$ is invariant by induction.
\end{proof}

\textit{Remark}.
Our prior work also establishes standard considerations such as e.g. (Lipschitz) continuity \cite{sabelhaus_safe_2022}.

\begin{figure*}[tb]
    \centering
    \includegraphics[width=\textwidth,height=5.5cm]{figures/foot_height_final.pdf}
    \caption{Feedback control test of Horton lifting its front leg. The test's four stages (a)-(d) demonstrate recovery from a human disturbance. Foot height (red dot distance from testbed surface) converges when the robot is undisturbed, showing dynamic balancing. Representative snapshots correspond to steady-state operation during each stage.}
    \label{fig:horton_foot_height}
    \vspace{-0.4cm}
\end{figure*}

% The figure shows the foot height of Horton's lifted front leg during the experiment. The foot height is the distance from the center of the red dot mark to the surface of our testbed. We artificially divide the process into four stages (a)-(d). A typical snapshot of Horton's posture at each stage is presented above.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Pose Controller}

The preceding sections establish the safety of actuator states for any choice of pose controller $\bv(\bz(k))$.
For tests in this article, we use proportional-integral controllers with anti-windup (PIAW) to track a bending angle for each limb of the $J$-many limbs.
To do so, with limb angles as pose states $\bq = \begin{bmatrix} \theta_1 & \hdots & \theta_J \end{bmatrix}^\top$ and target angles as $\bar \bq$, define the error in each limb pose as $\delta_i(k) \defeq \theta_i(k) - \bar\theta_i(k)$.

For the control, group the $j$-th limb's two SMAs into one antagonistic pair as in prior work \cite{patterson_robust_2022,sabelhaus_safe_2022}, forming a single input $\mu_j \in [-1, 1]$ by mapping positive duty cycles to one actuator and negative to the other:

\vspace{-0.3cm}
\begin{align}
    v_{2i} & = \mu_j, \quad v_{2i+1} = 0 \quad \text{if} \; \mu_j \geq 0, \notag \\
    v_{2i} & = 0, \quad v_{2i+1} = -\mu_j \quad \text{if} \; \mu_j < 0. \notag
\end{align}

\noindent Then, dropping indexing, take $\mu$ as saturated output from a commanded signal $\eta$ as $\mu = \text{sat}(\eta)$.
The scalar PIAW controllers are then defined in terms of $\eta$, with sampling time $\Delta_t$, as

\vspace{-0.7cm}
\begin{align}
    \eta(\delta(k)) & = K_P \delta(k) + K_I \Delta_t \sum_{\tau=0}^{k-1} [\delta(\tau) \hdots \notag \\ 
    & + K_A (\mu(\tau-1) - \eta(\tau-1))]
\end{align}

\noindent The anti-windup term $(\mu-\eta)$ compensates for saturation.
All gains for experiments in this article were tuned as in our prior work \cite{sabelhaus_-situ_2022, sabelhaus_safe_2022}, and $\gamma=0.2$.
However, we used $K_A=0.0$ so although anti-windup was not operated in practice, it is implemented as a feature of our framework that was key to prior results \cite{patterson_robust_2022,sabelhaus_safe_2022}.



% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=\textwidth,height=5.5cm]{figures/foot_height_v5.pdf}
%     \caption{}
%     \label{fig:horton_foot_height}
% \end{figure*}

% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=\textwidth,height=7.4cm]{figures/horton_state_v3.pdf}
%     \caption{}
%     \label{fig:horton_state}
% \end{figure*}

% \begin{enumerate}
%     \item constraints and optimization?
%     \item PI and anti-windup
%     \item Saturating Controller
% \end{enumerate}

% \subsection{An example - Temperature model and the temperature supervisor}
% \begin{enumerate}
%     \item First order SMA temperature model
%     \item Temperature supervisor
% \end{enumerate}

==> Horton Balancing Paper ICRA 2023 arxiv/P4_Results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{0.1cm}
\section{Balancing with Temperature Supervisor}

% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=\textwidth,height=5.5cm]{figures/foot_height_v5.pdf}
%     \caption{}
%     \label{fig:horton_foot_height}
% \end{figure*}

We validate Horton's pose feedback and safety-guaranteed control framework together in a balancing test with a human disturbance.
This test mimics an unknown environmental contact that may occur in future locomotion.

\begin{figure*}[tb]
    \centering
    \includegraphics[width=\textwidth,height=7.4cm]{figures/horton_state_final_v2.pdf}
    \caption{Data recorded during the balancing test from Fig. \ref{fig:horton_foot_height} include (a) the limb bending angles $\bq = [\theta_1, \; \hdots, \; \theta_5]^\top$ and corresponding setpoints, (b) the ten SMAs temperature readings $\bx$ and limit $T^{MAX}$, and (c) control inputs of PWM duty cycles $\hat\bu$ as a percent. The two highlighted SMAs in (b) and (c) show the action of the safety supervisor.}
    \label{fig:horton_state}
    \vspace{-0.4cm}
\end{figure*}

% Data recorded during the balancing test in Fig. \ref{fig:horton_foot_height} include (a) the limb bending angles $\bq = \begin{bmatrix}\theta_1 & \hdots & \theta_5\end{bmatrix}^\top$ and corresponding setpoints, (b) the ten SMAs temperature readings and limit $T^{MAX}$, of SMA  and temperature readings of all 10 SMAs. 3 of 10 SMAs are highlighted in both (b) and (c) for analysis in the \textit{Results}  section. (c) The PWM output (in percentage) that applied to each SMA during the experiment.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experimental Design}

% To validate the design of Horton and the safe-guaranteed control framework, we establish experimental procedures that involve a balancing task under human interference. 

We developed a trajectory of setpoint angles $\bar\bq$ through manual experimentation that corresponded with the front leg ($L_1$) lifting off the ground.
% In the experiment, Horton needs to balance itself with the front leg ($L_1$) raised by following a preset trajectory. 
In the experiment, Horton was allowed to move unencumbered from its start position (Fig. \ref{fig:horton_foot_height}(a)), with a wait until it converged to one balancing pose (Fig. \ref{fig:horton_foot_height}(b)).
Then, a human disturbance (a hand pushing the robot down) intervenes and temporarily makes some setpoint angles infeasible (Fig. \ref{fig:horton_foot_height}(c)). 
% Horton is then trying to restore the predefined balancing stance without overheating any SMA. 
Finally, the human disturbance is removed and the feedback controller recovers Horton to the balancing state (Fig. \ref{fig:horton_foot_height}(d)). 
For verification of balancing in addition to the convergence of our bending sensor readings, we attached a red dot sticker to Horton's front foot to track its height, with time series data obtained from post-processing a video recording.
% Control constants were $K_p=1e^{-3}, K_I=5e^{-8}, \gamma=0.2$.
% Lastly, $K_A=0.0$ and so anti-windup is not used in this test, though it is implemented as a feature of our framework key to prior results \cite{patterson_robust_2022,sabelhaus_safe_2022}.

% . Typical snapshots of all steps in the above processes are shown correspondingly in Fig. \ref{fig:horton_foot_height}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Results}
% In this section, we include the result from a test on Horton that follows the preceding procedures. 

The feedback control test took 130 seconds in total to perform self-balancing, safety of actuator states under human disturbance, and recovery. 
% The experiment demonstrates the effectiveness of our supervisory control method in the soft legged robot's balancing task. 
Fig. \ref{fig:horton_foot_height} shows the height of the lifted front foot from the ground during the experiment. 
In the first balancing stage, the front foot's height converged to approximately 8.5 mm, with small oscillations due to noise.
% oscillated between 0.8 to 1.45 cm. 
The human's hand caused a large interference with leg $L_3$, raising the front foot up to 39.5 mm. 
Finally, the foot height returned to around 13.5 mm in the recovery stage, and was maintained for more than 30 seconds. 
The average balancing foot height of 11.9 mm is approximately 15\% of the robot's height, considered large versus past work on rigid robots \cite{park_finite-state_2013}.
% The data indicates the consistency of two balancing stages and the repeatability of our balancing movement under massive external disturbance.

% Note: during the end of the balancing phase, 0.85 cm 
% Kp = 0.008, Ki = 5e-8, Ka = 0.0, gamma = 0.2.
% Spine SMA was almost 25\% longer than the leg SMA, 51 mm versus 63 mm, 63/51 = 1.24. So the calibration is definitely off.

The safety supervisor successfully constrained actuator states during the test, as shown in experimental data for bending angles $\bq = [\theta_1, \; \hdots, \; \theta_5]^\top$, SMA temperatures $\bx = [T_1, \; \hdots, \; T_{10}]^\top$, and control inputs $\hat\bu = [u_1, \; \hdots, \; u_{10}]$ (Fig. \ref{fig:horton_state}).
Limbs $L_1$ and $L_2$ converged quickly to their specified setpoint, as did spine $S_2$, albeit with some steady-state error as it was forced to bend when the robot's center of gravity shifted.
In contrast, spine $S_1$ was commanded to an infeasible pose: at $T^{MAX}$, its SMA wires could not provide enough force to fully counter the gravitational load of the front leg.
As a result, the safety supervisor activated for the $S_1$- actuator, which remained below $T^{MAX}$ throughout the test (Fig. \ref{fig:horton_state}(b), blue line).
Similarly, the human disturbance caused supervisor activation for the $L_3+$ actuator from 40-77 sec., which remained around $T^{MAX}$ with some chatter before the robot was released (Fig. \ref{fig:horton_state}(b), orange line).
This experiment demonstrates the effectiveness of our supervisory control method.

% Fig. \ref{fig:horton_state} contains robot bending angles $\bq = \begin{bmatrix}\theta_1 & \hdots & \theta_5\end{bmatrix}^\top$, temperature readings of SMAs $\bx = \begin{bmatrix} T_1 & \hdots & T_{10} \end{bmatrix}^\top$ , and corresponding output PWM percentage for all SMAs $\bu = \begin{bmatrix} u_1 & \hdots & u_{10}\end{bmatrix}^\top$. 
% All limbs were tracking the setpoints reasonably well expect $S_1$ (Fig. \ref{fig:horton_state}(a)). 

% The spine $S_1$ was required to lift both $L_1$ and itself during the balancing and soon overheated and triggered the temperature supervisor. 
% The blue lines show the temperature of $S_1$ stayed beyond the temperature limit and the output of the SMA was limited to the maximum output under safety constraints (Fig. \ref{fig:horton_foot_height}(b)(c)). 
% As human disturbance intervened, the state error of $L_3$ increased and overheated the limb. 
% The orange lines between 40-77s indicate that the supervisor held the SMA under safe temperature with insignificantly chattering (Fig. \ref{fig:horton_foot_height}(b)(c)). 
% $S_2$ had a relatively large steady-state error during the experiment since it naturally bent to the opposite direction as the center of gravity shifted. 

% Contains: 
% \begin{enumerate}
% \item(a) screenshots of Horton's posture of different stages - settled - balancing - disturbed - recovery
% \item(b) solid - actual angle of each limb, dashed - reference of each limb
% \item(c) temperature, PWM of each limbs \hl{\textbf{TBD}}
% \end{enumerate}
% \subsection{Evaluation}






==> Horton Balancing Paper ICRA 2023 arxiv/P5_Discussion_and_Conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion and Conclusion}
This paper demonstrates for the first time a soft legged robot with full pose control and verifiable safety on aspects of its operation. 
Horton is capable of dynamic balancing on two of its three legs, and maintaining safe operation during disturbances. 
This progress toward dynamic, controlled soft legged locomotion could significantly expand robotic exploration of unknown environments.
The safety framework is applicable to many other legged soft robots with actuator dynamics.
% This marks progress towards the practical implementation of mobile soft robots for expanding exploration capabilities in unstructured environments.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Limitations}

The balancing test confirms the safety specification for Horton's $S_1$- spine actuator.
However, chatter in $L_3+$ shows some temperatures slightly above $T_{MAX}$.
This is expected, as the supervisor's predictions use the thermal dynamics model (eqn. (\ref{eqn:umax})) which was not recalibrated per-SMA.
The spines' wires are 25\% longer than the legs' wires, so imprecise model parameters are the likely cause, which does not indicate theoretical issues.
% , and does not affect this article's fundamental contribution.

The balancing test showed the robot maintaining a lifted leg in otherwise-unstable poses.
However, though the pose controller converged to the same values of $\bq$ both before and after the disturbance (Fig. \ref{fig:horton_state}(a)), the foot height converged to a different value (Fig. \ref{fig:horton_foot_height}).
This is also expected, since the constant curvature assumption does not hold for Horton's limbs (c.f. Fig. \ref{fig:horton_balancing} vs. Fig. \ref{fig:horton_hardware_and_system_architecture}(d)), and confirms that our choice of state space does not uniquely determine its kinematics.
Future work will focus on alternative representations for $\bq$.
We emphasize this article's contribution as proof-of-concept for safety in any balancing motion.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Future Work}

Hardware designs, including the planar limbs and tether, were motivated by this article's focus on fundamental control results.
Future work seeks to design a Horton robot for practical locomotion, untethered, in 3D.
Design modifications will reduce weight and power needs by drawing from past work \cite{Huang2019}.
Stiffer materials (and additional SMA wires) could produce motions more consistent with the constant-curvature assumption.
This may allow safe control algorithms to be extended to the robot's pose in addition to its actuators.

% In future work, several design modifications will be made to increase the actuation power and decrease overall weight. Additional SMAs can be incorporated into each limb and ridges beyond those necessary for constraining motion to bidirectional bending will be removed. 

%plan to modify the limb design by removing the ridges on its flat surface, thereby reducing the extra weight on Horton. To in
% The limb design can be modified by removing the ridges on the flat surface. This should reduce the obstacles caused by the extra weight on the limbs and overcome the material stiffness, thereby making it easier for Horton to lift itself and walk untethered.

% \fix{actually walk, remove tether}

% This control framework has the potential to be adapted to a variety of soft robotic applications that could benefit from the high work density of SMAs, now with additional safety guarantees. 



% \addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
%                                   % on the last page of the document manually. It shortens
%                                   % the textheight of the last page by a suitable amount.
%                                   % This command does not take effect until the next page
%                                   % so it should come on the page before the last. Make
%                                   % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
